Role of Transients in Two-Bounce Non-Line-of-Sight Imaging

The goal of non-line-of-sight (NLOS) imaging is to image objects occluded from the camera's field of view using multiply scattered light. Recent works have demonstrated the feasibility of two-bounce (2B) NLOS imaging by scanning a laser and measuring cast shadows of occluded objects in scenes with two relay surfaces. In this work, we study the role of time-of-flight (ToF) measurements, \ie transients, in 2B-NLOS under multiplexed illumination. Specifically, we study how ToF information can reduce the number of measurements and spatial resolution needed for shape reconstruction. We present our findings with respect to tradeoffs in (1) temporal resolution, (2) spatial resolution, and (3) number of image captures by studying SNR and recoverability as functions of system parameters. This leads to a formal definition of the mathematical constraints for 2B lidar. We believe that our work lays an analytical groundwork for design of future NLOS imaging systems, especially as ToF sensors become increasingly ubiquitous.

==> tables/comparison_table.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}m{#1}}

\def\red{red!20}
\def\green{green!20}
\def\yellow{yellow!30}
\def\gray{gray!20}

\begin{table*}%[htbp]
\centering
\setlength{\extrarowheight}{0pt}
\addtolength{\extrarowheight}{\aboverulesep}
\addtolength{\extrarowheight}{\belowrulesep}
\setlength{\aboverulesep}{0pt}
\setlength{\belowrulesep}{0pt}

\begin{NiceTabular}{*{1}{P{0.16\linewidth}}*{1}{P{0.14\linewidth}}*{1}{P{0.07\linewidth}}*{1}{P{0.07\linewidth}}*{1}{P{0.1\linewidth}}*{1}{P{0.1\linewidth}}*{1}{P{0.12\linewidth}}}[hvlines]

\Block{2-1}{\textbf{NLOS Imaging Domain}} & \multicolumn{3}{c}{\textbf{Key Components}} & \multicolumn{3}{c}{\textbf{Key Features}} \\

&  \cellcolor{\gray} \textbf{Assisting Surfaces} & \cellcolor{\gray} \textbf{Sensor Type} & \cellcolor{\gray} \textbf{Light Source} & \cellcolor{\gray} \textbf{Number of Captures} & \cellcolor{\gray} \textbf{Recovered Dimensions} & \cellcolor{\gray} \textbf{Signal Quality} \\

\Block[fill=\gray]{2-1}{\textbf{Passive Occlusion-Aided}\cite{saunders2019computational,sharma2021you, bouman2017turning}} & Relay Wall/Floor & \Block{2-1}{Intensity} & \Block{2-1}{Passive} & \Block[fill=\green]{2-1}{Low} & \Block[fill=\red]{2-1}{2D} & \Block[fill=\red]{2-1}{Low (strong background)} \\

 & Edge Occluders & & & & &  \\

\Block[fill=\gray]{2-1}{\textbf{Three-Bounce Transient} \cite{kirmani2009looking, o2018confocal, xin2019theory, rapp2020seeing}}  & Relay Wall/Floor & \Block{2-1}{ToF} & \Block{2-1}{Active (Scan)} & \Block[fill=\red]{2-1}{High} & \Block[fill=\green]{2-1}{3D} & \Block[fill=\yellow]{2-1}{Medium (3-bounce)} \\

 & Edge Occluders & & & & & \\


\cellcolor{\gray} \textbf{Two-Bounce Transient (Ours)} & Two LOS Walls & ToF & Active (Flash) & \cellcolor{\green} Low & \cellcolor{\green} 3D & \cellcolor{\green} High (2-bounce) \\

\end{NiceTabular}

\caption{\textbf{Comparison of NLOS Methods.} Passive approaches require fewer measurements but can either recover up to two dimensions or are strongly affected by ambient noise. Works exploiting three-bounce light paths demonstrate 3D imaging around the corner but require a bounce on the hidden surface, reducing the signal quality. We analyze exploiting two-bounce transients for NLOS imaging. }
\label{table2}
\end{table*}
